Photon and di-photon production at ATLAS

The latest ATLAS measurements of the cross section for the inclusive production of isolated prompt photons in $pp$ collisions at a centre-of-mass energy $\sqrt{s}$ = 7 TeV at the LHC are presented, as well as the measurement of the di-photon production cross section.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = delmastro

default: latex

# lxplus fix:
# export PATH=/afs/cern.ch/sw/XML/texlive/latest/bin/x86_64-linux:$PATH

latex:
	latex  ${BASENAME}
	latex  ${BASENAME}
	#bibtex ${BASENAME}
	#latex  ${BASENAME}
	#latex  ${BASENAME}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp *.spl

binclean:
	rm -f ${BASENAME}.pdf

